Pandemic Pressures and Public Health Care: Evidence from England

This paper documents that the COVID-19 pandemic induced pressures on the health care system have significant adverse knock-on effects on the accessibility and quality of non-COVID-19 care. We observe persistently worsened performance and longer waiting times in A&E; drastically limited access to specialist care; notably delayed or inaccessible diagnostic services; acutely undermined access to and quality of cancer care. We find that providers under COVID-19 pressures experience notably more excess deaths among non-COVID related hospital episodes such as, for example, for treatment of heart attacks. We estimate there to be at least one such non-COVID-19 related excess death among patients being admitted to hospital for non-COVID-19 reasons for every 30 COVID-19 deaths that is caused by the disruption to the quality of care due to COVID-19. In total, this amounts to 4,003 non COVID-19 excess deaths from March 2020 to February 2021. Further, there are at least 32,189 missing cancer patients that should counterfactually have started receiving treatment which suggests continued increased numbers of excess deaths in the future due to delayed access to care in the past.

==> fragment-absence-vaccination-hospital_cases-nhsboostervaxxerate.tex <==
log(COVID-19 cases in hospital$_t$)&       0.007***&       0.005***&       0.006***&       0.010***&       0.001   &       0.000   \\
                    &     (0.002)   &     (0.002)   &     (0.002)   &     (0.003)   &     (0.001)   &     (0.002)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases in hospital$_t$)&      -0.005** &      -0.003   &      -0.005** &      -0.009** &       0.000   &      -0.000   \\
                    &     (0.003)   &     (0.002)   &     (0.003)   &     (0.004)   &     (0.002)   &     (0.004)   \\
\addlinespace Observations&        2248   &        2139   &        2139   &        2139   &        2139   &        2139   \\
Clusters            &         126   &         122   &         122   &         122   &         122   &         122   \\


==> fragment-absence-vaccination-hospital_cases-nhsfullyvaxxrate.tex <==
log(COVID-19 cases in hospital$_t$)&       2.109***&       1.773***&       2.144***&       3.373***&       0.341   &       0.383   \\
                    &     (0.544)   &     (0.522)   &     (0.570)   &     (0.798)   &     (0.495)   &     (0.732)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases in hospital$_t$)&      -1.927***&      -1.543***&      -1.993***&      -3.155***&      -0.212   &      -0.367   \\
                    &     (0.586)   &     (0.560)   &     (0.619)   &     (0.867)   &     (0.542)   &     (0.797)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination-hospital_cases-nhsvaxxrate.tex <==
log(COVID-19 cases in hospital$_t$)&       2.681***&       2.253***&       2.734***&       4.285***&       0.485   &       0.572   \\
                    &     (0.699)   &     (0.672)   &     (0.727)   &     (1.021)   &     (0.629)   &     (0.929)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases in hospital$_t$)&      -2.482***&      -2.010***&      -2.565***&      -4.035***&      -0.359   &      -0.557   \\
                    &     (0.734)   &     (0.704)   &     (0.769)   &     (1.080)   &     (0.668)   &     (0.985)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination-new_admissions-nhsboostervaxxerate.tex <==
log(New COVID-19 admissions$_t$)&       0.007***&       0.006** &       0.006***&       0.010***&       0.002   &      -0.001   \\
                    &     (0.002)   &     (0.002)   &     (0.002)   &     (0.003)   &     (0.002)   &     (0.003)   \\
NHS Vaccination Uptake $\times$ log(New COVID-19 admissions$_t$)&      -0.003   &      -0.002   &      -0.004   &      -0.006   &       0.001   &       0.002   \\
                    &     (0.004)   &     (0.003)   &     (0.004)   &     (0.005)   &     (0.003)   &     (0.005)   \\
\addlinespace Observations&        2248   &        2139   &        2139   &        2139   &        2139   &        2139   \\
Clusters            &         126   &         122   &         122   &         122   &         122   &         122   \\


==> fragment-absence-vaccination-new_admissions-nhsfullyvaxxrate.tex <==
log(New COVID-19 admissions$_t$)&       1.943***&       1.605** &       2.196***&       3.057***&       0.627   &       0.358   \\
                    &     (0.727)   &     (0.724)   &     (0.762)   &     (1.016)   &     (0.691)   &     (0.947)   \\
NHS Vaccination Uptake $\times$ log(New COVID-19 admissions$_t$)&      -1.608** &      -1.243   &      -1.887** &      -2.600** &      -0.402   &      -0.228   \\
                    &     (0.792)   &     (0.788)   &     (0.837)   &     (1.122)   &     (0.765)   &     (1.046)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination-new_admissions-nhsvaxxrate.tex <==
log(New COVID-19 admissions$_t$)&       2.471***&       2.051** &       2.806***&       3.866***&       0.859   &       0.494   \\
                    &     (0.933)   &     (0.930)   &     (0.972)   &     (1.299)   &     (0.873)   &     (1.205)   \\
NHS Vaccination Uptake $\times$ log(New COVID-19 admissions$_t$)&      -2.124** &      -1.684*  &      -2.484** &      -3.386** &      -0.639   &      -0.367   \\
                    &     (0.989)   &     (0.985)   &     (1.037)   &     (1.389)   &     (0.937)   &     (1.291)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination-occupied_mv_beds-nhsboostervaxxerate.tex <==
log(COVID-19 cases on ventilators$_t$)&       0.003** &       0.003** &       0.007***&       0.011***&       0.000   &       0.001   \\
                    &     (0.002)   &     (0.002)   &     (0.002)   &     (0.003)   &     (0.002)   &     (0.003)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases on ventilators$_t$)&      -0.000   &      -0.002   &      -0.007** &      -0.012** &      -0.000   &      -0.002   \\
                    &     (0.003)   &     (0.003)   &     (0.003)   &     (0.005)   &     (0.003)   &     (0.004)   \\
\addlinespace Observations&        2248   &        2139   &        2139   &        2139   &        2139   &        2139   \\
Clusters            &         126   &         122   &         122   &         122   &         122   &         122   \\


==> fragment-absence-vaccination-occupied_mv_beds-nhsfullyvaxxrate.tex <==
log(COVID-19 cases on ventilators$_t$)&       0.519   &       0.312   &       1.504** &       2.693***&      -0.208   &       0.021   \\
                    &     (0.497)   &     (0.477)   &     (0.603)   &     (0.837)   &     (0.516)   &     (0.750)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases on ventilators$_t$)&      -0.237   &       0.004   &      -1.343** &      -2.455***&       0.303   &       0.083   \\
                    &     (0.551)   &     (0.530)   &     (0.670)   &     (0.935)   &     (0.575)   &     (0.838)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination-occupied_mv_beds-nhsvaxxrate.tex <==
log(COVID-19 cases on ventilators$_t$)&       0.706   &       0.444   &       1.977** &       3.462***&      -0.130   &       0.073   \\
                    &     (0.654)   &     (0.632)   &     (0.785)   &     (1.084)   &     (0.659)   &     (0.959)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases on ventilators$_t$)&      -0.431   &      -0.139   &      -1.809** &      -3.204***&       0.209   &       0.024   \\
                    &     (0.703)   &     (0.681)   &     (0.844)   &     (1.170)   &     (0.711)   &     (1.035)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2224   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-absence-vaccination.tex <==
log(New COVID-19 admissions$_t$)&       1.943***&       1.605** &       2.196***&               &               &               &               &               &               &       2.471***&       2.051** &       2.806***&               &               &               &               &               &               \\
                    &     (0.727)   &     (0.724)   &     (0.762)   &               &               &               &               &               &               &     (0.933)   &     (0.930)   &     (0.972)   &               &               &               &               &               &               \\
NHS Vaccination Uptake $\times$ log(New COVID-19 admissions$_t$)&      -1.608** &      -1.243   &      -1.887** &               &               &               &               &               &               &      -2.124** &      -1.684*  &      -2.484** &               &               &               &               &               &               \\
                    &     (0.792)   &     (0.788)   &     (0.837)   &               &               &               &               &               &               &     (0.989)   &     (0.985)   &     (1.037)   &               &               &               &               &               &               \\
log(COVID-19 cases in hospital$_t$)&               &               &               &       2.109***&       1.773***&       2.144***&               &               &               &               &               &               &       2.681***&       2.253***&       2.734***&               &               &               \\
                    &               &               &               &     (0.544)   &     (0.522)   &     (0.570)   &               &               &               &               &               &               &     (0.699)   &     (0.672)   &     (0.727)   &               &               &               \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases in hospital$_t$)&               &               &               &      -1.927***&      -1.543***&      -1.993***&               &               &               &               &               &               &      -2.482***&      -2.010***&      -2.565***&               &               &               \\
                    &               &               &               &     (0.586)   &     (0.560)   &     (0.619)   &               &               &               &               &               &               &     (0.734)   &     (0.704)   &     (0.769)   &               &               &               \\
log(COVID-19 cases on ventilators$_t$)&               &               &               &               &               &               &       0.519   &       0.312   &       1.504** &               &               &               &               &               &               &       0.706   &       0.444   &       1.977** \\
                    &               &               &               &               &               &               &     (0.497)   &     (0.477)   &     (0.603)   &               &               &               &               &               &               &     (0.654)   &     (0.632)   &     (0.785)   \\
NHS Vaccination Uptake $\times$ log(COVID-19 cases on ventilators$_t$)&               &               &               &               &               &               &      -0.237   &       0.004   &      -1.343** &               &               &               &               &               &               &      -0.431   &      -0.139   &      -1.809** \\
                    &               &               &               &               &               &               &     (0.551)   &     (0.530)   &     (0.670)   &               &               &               &               &               &               &     (0.703)   &     (0.681)   &     (0.844)   \\
\addlinespace Observations&        2248   &        2224   &        2224   &        2248   &        2224   &        2224   &        2248   &        2224   &        2224   &        2248   &        2224   &        2224   &        2248   &        2224   &        2224   &        2248   &        2224   &        2224   \\
Clusters            &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   &         126   \\


==> fragment-ae_statistics-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&       0.019   &       0.019   &       2.351***&       1.105***&       0.076***\\
                    &     (0.012)   &     (0.012)   &     (0.475)   &     (0.210)   &     (0.025)   \\
Staff Absence Rate$_t$&       0.096   &       0.701   &     110.462***&      31.700** &       2.389*  \\
                    &     (0.566)   &     (0.542)   &    (29.971)   &    (13.952)   &     (1.264)   \\
\addlinespace Mean of DV&     8720.04   &     2798.45   &       18.61   &        4.74   &        0.11   \\
Observations        &        2258   &        2258   &        2257   &        2257   &        2257   \\
Clusters            &         127   &         127   &         127   &         127   &         127   \\


==> fragment-ae_statisticslognew_cases-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&       0.019   &       0.007   &       2.110***&       1.072***&       0.059** \\
                    &     (0.012)   &     (0.009)   &     (0.509)   &     (0.229)   &     (0.028)   \\
Staff Absence Rate$_t$&       0.096   &       0.400   &     128.792***&      41.127***&       2.630** \\
                    &     (0.566)   &     (0.512)   &    (28.336)   &    (14.091)   &     (1.328)   \\
\addlinespace Mean of DV&     8720.04   &     2877.27   &       19.01   &        4.93   &        0.12   \\
Observations        &        2258   &        2153   &        2153   &        2153   &        2153   \\
Clusters            &         127   &         123   &         123   &         123   &         123   \\


==> fragment-aeattendances-hospital_cases.tex <==
confirmed COVID-19 patients in hospital&      -0.020   &      -0.027   &       6.857***&      42.964***&      -0.051*  \\
                    &     (0.016)   &     (0.018)   &     (2.027)   &     (7.169)   &     (0.026)   \\
\addlinespace Mean of DV&           9   &           9   &         151   &         447   &           7   \\
Observations        &        2776   &        2609   &        2747   &        2747   &        2747   \\
Clusters            &         172   &         153   &         170   &         170   &         170   \\


==> fragment-aeattendances-new_admissions.tex <==
New COVID-19 hospital admissions&      -0.012   &      -0.013   &       5.447***&      54.661***&      -0.031   \\
                    &     (0.015)   &     (0.016)   &     (1.428)   &     (6.966)   &     (0.021)   \\
\addlinespace Mean of DV&           9   &           9   &         151   &         447   &           7   \\
Observations        &        2776   &        2609   &        2747   &        2747   &        2747   \\
Clusters            &         172   &         153   &         170   &         170   &         170   \\


==> fragment-aeattendances-new_cases.tex <==
COVID-19 cases      &      -0.009*  &      -0.005   &       2.250   &      23.162***&      -0.007   \\
                    &     (0.005)   &     (0.005)   &     (1.756)   &     (7.322)   &     (0.010)   \\
\addlinespace Mean of DV&           9   &           9   &         171   &         508   &           7   \\
Observations        &        2154   &        2154   &        2154   &        2154   &        2154   \\
Clusters            &         122   &         122   &         122   &         122   &         122   \\


==> fragment-aeattendances-occupied_mv_beds.tex <==
\# of COVID-19 cases in ventilator beds&       0.022** &       0.020*  &       3.628***&      34.526***&       0.024*  \\
                    &     (0.011)   &     (0.011)   &     (0.970)   &     (4.889)   &     (0.013)   \\
\addlinespace Mean of DV&           9   &           9   &         151   &         447   &           7   \\
Observations        &        2776   &        2609   &        2747   &        2747   &        2747   \\
Clusters            &         172   &         153   &         170   &         170   &         170   \\


==> fragment-cancer-sa_rate-new_admissions.tex <==
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&      -0.018   &      -0.031***&      -0.024** &       0.148   &       0.363*  &       1.250** \\
                    &     (0.014)   &     (0.011)   &     (0.009)   &     (0.400)   &     (0.184)   &     (0.509)   \\
Staff Absence Rate $_{t-1}^t$&      -0.370   &       0.220   &       0.830   &      36.909   &       1.987   &      48.150   \\
                    &     (0.961)   &     (0.816)   &     (0.700)   &    (32.256)   &    (14.584)   &    (36.025)   \\
\addlinespace Mean of DV&      116.32   &       15.67   &        8.55   &        8.86   &        4.03   &       28.98   \\
Observations        &       28090   &       26146   &       26158   &       25671   &       24586   &       24103   \\
Clusters            &         127   &         127   &         126   &         127   &         127   &         125   \\


==> fragment-cancerlognew_cases-sa_rate-new_admissions.tex <==
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&      -0.012   &      -0.021*  &      -0.020*  &       0.357   &       0.234   &       1.584** \\
                    &     (0.014)   &     (0.012)   &     (0.010)   &     (0.461)   &     (0.201)   &     (0.620)   \\
Staff Absence Rate $_{t-1}^t$&      -0.285   &       0.325   &       1.049   &      40.707   &       0.198   &      47.551   \\
                    &     (0.971)   &     (0.826)   &     (0.709)   &    (32.906)   &    (14.610)   &    (36.445)   \\
\addlinespace Mean of DV&      117.46   &       15.79   &        8.63   &        8.92   &        4.04   &       29.00   \\
Observations        &       27392   &       25448   &       25470   &       25031   &       23952   &       23526   \\
Clusters            &         123   &         123   &         123   &         123   &         123   &         123   \\


==> fragment-diagnostic-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&      -0.030   &               &               &               &               \\
                    &     (0.023)   &               &               &               &               \\
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&               &       0.010   &       0.048** &       0.554   &       2.136** \\
                    &               &     (0.013)   &     (0.022)   &     (0.627)   &     (0.926)   \\
Staff Absence Rate$_t$&      -3.115** &               &               &               &               \\
                    &     (1.501)   &               &               &               &               \\
Staff Absence Rate $_{t-1}^t$&               &       1.844   &       0.731   &      72.950   &      32.807   \\
                    &               &     (1.175)   &     (2.183)   &    (58.187)   &    (92.872)   \\
\addlinespace Mean of DV&      874.54   &        5.61   &        3.97   &       31.72   &       17.48   \\
Observations        &       30305   &       27702   &        2246   &       27702   &        2246   \\
Clusters            &         127   &         127   &         127   &         127   &         127   \\


==> fragment-diagnosticlognew_cases-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&      -0.025   &               &               &               &               \\
                    &     (0.027)   &               &               &               &               \\
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&               &       0.003   &       0.059** &       0.141   &       2.654** \\
                    &               &     (0.017)   &     (0.029)   &     (0.773)   &     (1.135)   \\
Staff Absence Rate$_t$&      -2.619*  &               &               &               &               \\
                    &     (1.462)   &               &               &               &               \\
Staff Absence Rate $_{t-1}^t$&               &       1.773   &       0.562   &      69.353   &      33.287   \\
                    &               &     (1.197)   &     (2.239)   &    (59.281)   &    (94.149)   \\
\addlinespace Mean of DV&      898.73   &        5.60   &        3.94   &       31.65   &       17.26   \\
Observations        &       28884   &       26568   &        2142   &       26568   &        2142   \\
Clusters            &         123   &         123   &         123   &         123   &         123   \\


==> fragment-rtt-.tex <==
log(COVID-19 cases in catchment area$_t$)&      -0.008***&      -0.024***&      -0.010***&               &               &               &       0.001   &               &               \\
                    &     (0.003)   &     (0.005)   &     (0.004)   &               &               &               &     (0.001)   &               &               \\
log($\sum_{t-1}^t$ COVID-19 cases in catchment area$_t$ )&               &               &               &      -0.002   &      -0.003   &      -0.001   &               &       0.000   &               \\
                    &               &               &               &     (0.003)   &     (0.004)   &     (0.002)   &               &     (0.001)   &               \\
log($\sum_{t-2}^t$ COVID-19 cases in catchment area$_t$ )&               &               &               &               &               &               &               &               &      -0.001   \\
                    &               &               &               &               &               &               &               &               &     (0.001)   \\
\addlinespace Mean of DV&      586.66   &       98.41   &      391.49   &     2602.38   &    47501.17   &       15.59   &        0.77   &        0.60   &        0.46   \\
Observations        &      158045   &      127545   &      156399   &      159868   &      159863   &      159863   &      159868   &      159868   &      159868   \\
Clusters            &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   \\


==> fragment-rtt-new_cases.tex <==
log(COVID-19 cases in catchment area$_t$)&      -0.008***&      -0.024***&      -0.010***&               &               &               &       0.001   &               &               \\
                    &     (0.003)   &     (0.005)   &     (0.004)   &               &               &               &     (0.001)   &               &               \\
log($\sum_{t-1}^t$ COVID-19 cases in catchment area$_t$ )&               &               &               &      -0.002   &      -0.003   &      -0.001   &               &       0.000   &               \\
                    &               &               &               &     (0.003)   &     (0.004)   &     (0.002)   &               &     (0.001)   &               \\
log($\sum_{t-2}^t$ COVID-19 cases in catchment area$_t$ )&               &               &               &               &               &               &               &               &      -0.001   \\
                    &               &               &               &               &               &               &               &               &     (0.001)   \\
\addlinespace Mean of DV&      586.66   &       98.41   &      391.49   &     2602.38   &    47501.17   &       15.59   &        0.77   &        0.60   &        0.46   \\
Observations        &      158045   &      127545   &      156399   &      159868   &      159863   &      159863   &      159868   &      159868   &      159868   \\
Clusters            &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   \\


==> fragment-rtt-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&      -0.019   &      -0.062***&      -0.030   &               &               &               &       0.316   &               &               \\
                    &     (0.012)   &     (0.017)   &     (0.020)   &               &               &               &     (0.207)   &               &               \\
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&               &               &               &       0.006   &       0.016   &       0.010   &               &       0.724** &               \\
                    &               &               &               &     (0.010)   &     (0.016)   &     (0.008)   &               &     (0.319)   &               \\
log($\sum_{t-2}^t$ New COVID-19 admissions$_t$ )&               &               &               &               &               &               &               &               &       0.721** \\
                    &               &               &               &               &               &               &               &               &     (0.327)   \\
Staff Absence Rate$_t$&      -2.309** &      -4.239***&       0.546   &               &               &               &      47.150***&               &               \\
                    &     (0.980)   &     (1.277)   &     (1.533)   &               &               &               &    (14.758)   &               &               \\
Staff Absence Rate $_{t-1}^t$&               &               &               &       1.649*  &       3.006** &       1.340** &               &      85.749***&               \\
                    &               &               &               &     (0.878)   &     (1.274)   &     (0.616)   &               &    (27.752)   &               \\
Staff Absence Rate $_{t-2}^t$&               &               &               &               &               &               &               &               &     119.102***\\
                    &               &               &               &               &               &               &               &               &    (38.854)   \\
\addlinespace Mean of DV&      564.94   &       95.08   &      381.08   &     2512.81   &    45976.77   &       15.64   &       76.76   &       59.83   &       46.45   \\
Observations        &       35663   &       28626   &       35235   &       36062   &       36062   &       36062   &       36076   &       36062   &       36031   \\
Clusters            &         127   &         127   &         127   &         127   &         127   &         127   &         127   &         127   &         127   \\


==> fragment-rttlognew_cases-sa_rate-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&      -0.016   &      -0.060***&      -0.026   &               &               &               &       0.173   &               &               \\
                    &     (0.014)   &     (0.019)   &     (0.022)   &               &               &               &     (0.233)   &               &               \\
log($\sum_{t-1}^t$ New COVID-19 admissions$_t$ )&               &               &               &       0.005   &       0.012   &       0.007   &               &       0.414   &               \\
                    &               &               &               &     (0.012)   &     (0.019)   &     (0.009)   &               &     (0.365)   &               \\
log($\sum_{t-2}^t$ New COVID-19 admissions$_t$ )&               &               &               &               &               &               &               &               &       0.438   \\
                    &               &               &               &               &               &               &               &               &     (0.372)   \\
Staff Absence Rate$_t$&      -2.228** &      -4.106***&       0.671   &               &               &               &      46.497***&               &               \\
                    &     (1.003)   &     (1.300)   &     (1.543)   &               &               &               &    (14.938)   &               &               \\
Staff Absence Rate $_{t-1}^t$&               &               &               &       1.713*  &       3.043** &       1.315** &               &      83.499***&               \\
                    &               &               &               &     (0.885)   &     (1.273)   &     (0.620)   &               &    (27.768)   &               \\
Staff Absence Rate $_{t-2}^t$&               &               &               &               &               &               &               &               &     120.916***\\
                    &               &               &               &               &               &               &               &               &    (39.173)   \\
\addlinespace Mean of DV&      565.95   &       95.06   &      380.97   &     2516.34   &    45997.44   &       15.61   &       76.74   &       59.76   &       46.31   \\
Observations        &       34723   &       27884   &       34325   &       35117   &       35117   &       35117   &       35131   &       35117   &       35086   \\
Clusters            &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   &         123   \\


==> fragment-shmi-dlogexcess-new_cases.tex <==
log()               &       0.009***&       0.013***&       0.017***&       0.023***&       0.032***&       0.032***\\
                    &     (0.002)   &     (0.003)   &     (0.004)   &     (0.006)   &     (0.010)   &     (0.010)   \\
\addlinespace Observations&        2078   &        2078   &        2078   &        2078   &        2078   &        2078   \\
Clusters            &         123   &         123   &         123   &         123   &         123   &         123   \\


==> fragment-shmi-sa_rate-dchexcess-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&       3.418***&       4.495***&       4.371***&       4.146***&       4.533***\\
                    &     (1.291)   &     (1.301)   &     (1.320)   &     (1.278)   &     (1.310)   \\
Staff Absence Rate$_t$&     151.220*  &     194.554** &     183.822** &     189.352** &     114.806   \\
                    &    (88.333)   &    (87.422)   &    (86.510)   &    (86.025)   &   (101.629)   \\
\addlinespace Observations&        2202   &        2202   &        2173   &        2173   &        2173   \\
Clusters            &         124   &         124   &         123   &         123   &         123   \\


==> fragment-shmilognew_cases-sa_rate-dchexcess-new_admissions.tex <==
log(New COVID-19 admissions$_t$)&       2.323   &       3.701** &       3.760** &       3.530** &       4.486***\\
                    &     (1.497)   &     (1.526)   &     (1.556)   &     (1.529)   &     (1.587)   \\
Staff Absence Rate$_t$&     137.994   &     185.860** &     168.212*  &     173.734*  &     112.940   \\
                    &    (91.088)   &    (90.068)   &    (89.149)   &    (88.550)   &   (103.792)   \\
\addlinespace Observations&        2150   &        2150   &        2133   &        2133   &        2133   \\
Clusters            &         123   &         123   &         122   &         122   &         122   \\

